UFO: Chain-of-Evaluation for Omni-Condition Alignment in Multi-Modal Image Generation

Multi-modal image generation, particularly subject-driven customization, has garnered growing attention in recent years. Despite the rapid advancement of generative models, their evaluation remains largely lagging. Existing methods, whether embedding-based or Multi-modal Large Language Model (MLLM)-based, evaluate alignment with each modal condition in isolation, which contradicts the simultaneous condition alignment objective of multi-modal image generation, leading to poor consistency with human judgments. To address this challenge, we propose UFO, the first unified framework for omni-condition alignment simultaneous evaluation. Specifically, UFO introduces a novel Atomized Chain-of-Evaluation paradigm, i.e., it first decomposes omni-condition alignment into a sequential chain of fine-grained, disentangled Atomic Evaluation Units (AEUs), categorizes them into distinct modality-relevance classes, and then employs general or dedicated functional calls for accurate verification of different AEU types. Experimental results demonstrate that UFO achieves the highest correlation with human evaluation preferences, delivering an average improvement of 15.25%. Furthermore, we present UFO-Bench, a dedicated benchmark designed to holistically evaluate the performance of existing customization models under the diverse mutual interactions of textual and visual conditions.

==> check-anonymous.tex <==
\PassOptionsToClass{anonymous,fontB}{framexpaper}
\input{main.tex}


==> check-print.tex <==
\PassOptionsToClass{print,fontB}{framexpaper}
\input{main.tex}


==> cvpr.tex <==
% CVPR-inspired comparison: compact Times-style typography in one column.
% This is a branded design study, not an official CVPR submission class.
\def\fxcvprlayout{1}
\input{main.tex}


==> sections_pre/closing.tex <==
\fxkicker{Findings / limits / reproducibility}
\section{Conclusion}
Summarize what the evidence establishes and return to the research question from the introduction. Explain the practical consequence in concrete terms. Keep the conclusion proportional to the demonstrated scope and reserve implementation details for the method or appendix.
\subsection{Limitations}
Describe the settings that have not been evaluated, assumptions inherited from the training setup, and any known failure cases. Connect each limitation to its practical consequence so readers can judge whether the method is appropriate for their application.
\section*{Acknowledgments}
Replace this paragraph with the approved funding, contribution and resource acknowledgments. The class supports an anonymous mode that hides front-matter identity; remove identifying body text and document metadata separately for an actual review submission.
\begingroup\small
\bibliographystyle{plainnat}
\bibliography{references}
\endgroup
\appendix
\section{Reproducibility details}
\begin{table}[htbp]
\centering\small\renewcommand\arraystretch{1.22}
\begin{tabularx}{\linewidth}{@{}p{.30\linewidth}X@{}}
\toprule
\textbf{Item} & \textbf{Information to provide}\\\midrule
Model and data & Checkpoint identifiers, data versions and filtering policy.\\
Training configuration & Optimizer, learning rate, batch size and random seeds.\\
Evaluation & Prompts, metrics, sampling settings and hardware.\\
Release artifacts & Source code, configuration files and model access.\\\bottomrule
\end{tabularx}
\caption{A compact appendix table. Expand this shell with the details needed to reproduce the study.}
\end{table}
\vspace{2mm}
{\sffamily\fontsize{8}{11}\selectfont\color{FXMuted}
\textbf{About this specimen.} The title, author information and abbreviated scientific synopsis refer to Stream-R1. Writing prompts, simplified diagrams and placeholder tables were prepared for template review. This is an independent Frame-X design template for preprints and technical reports; a venue submission should use that venue's required class and formatting.}


==> sections_pre/experiments.tex <==
\fxkicker{Evidence / comparisons / analysis}
\section{Experiments}
\subsection{Experimental setup}
State the datasets, model checkpoints, resolution, sampling protocol, hardware and evaluation settings. Describe how prompts and random seeds are shared across comparisons. Report the unit for every efficiency measurement and distinguish latency from throughput. Table~\ref{tab:main} is a reusable results shell; dashes indicate values that have not been supplied.
\begin{table}[htbp]
\caption{Main comparison template. All entries are placeholders, not measured results. Replace the generic method names and metrics before publication.}\label{tab:main}
\centering\small\renewcommand{\arraystretch}{1.3}
\fxfitfigure{\begin{tabular}{@{}l D{.}{.}{2.2} D{.}{.}{2.2} D{.}{.}{2.1} D{.}{.}{2.0}@{}}
\toprule
\textbf{Method} & \multicolumn{1}{c}{\textbf{Quality $\uparrow$}} & \multicolumn{1}{c}{\textbf{Alignment $\uparrow$}} & \multicolumn{1}{c}{\textbf{FPS $\uparrow$}} & \multicolumn{1}{c}{\textbf{Steps $\downarrow$}}\\
\midrule
Teacher & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--}\\
Baseline A & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--}\\
Baseline B & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--} & \multicolumn{1}{r}{--}\\
\rowcolor{FXPale}\textbf{Proposed method} & \multicolumn{1}{r}{\textbf{--}} & \multicolumn{1}{r}{\textbf{--}} & \multicolumn{1}{r}{\textbf{--}} & \multicolumn{1}{r}{\textbf{--}}\\
\bottomrule
\end{tabular}}
\end{table}
\subsection{Ablation and visual analysis}
Change one component at a time, retain a matched evaluation budget and explain the expected effect. A good ablation connects the measured change to the proposed mechanism. Include uncertainty when it is supported by repeated measurements, and discuss cases that do not follow the main trend.
\begin{figure}[htbp]
\centering
\fxfitfigure{\begin{tikzpicture}[x=.77cm,y=.77cm,font=\sffamily\scriptsize]
\foreach \panel/\labeltext in {0/Frame 01,1/Frame 02,2/Frame 03}{
\begin{scope}[xshift=\panel*5.35cm]
\fill[FXPaper,rounded corners=2pt] (0,0) rectangle (6,3.4);
\foreach \x in {0,...,9}{\foreach \y in {0,...,3}{
\pgfmathtruncatemacro{\tone}{12+mod(\x*11+\y*17+\panel*29,76)}
\fill[FXTeal!\tone!FXPale,rounded corners=.5pt] (.3+\x*.54,.35+\y*.53) rectangle ++(.46,.45);
}}
\node[anchor=west,text=FXMuted] at (.3,2.93){\labeltext};
\draw[FXGold,line width=1pt] (2.0,.7) rectangle (3.5,2.3);
\end{scope}}
\end{tikzpicture}}
\caption{Synthetic saliency tiles for checking the green--teal--gold palette. The cells are decorative values, not model outputs; gold outlines demonstrate region annotations.}\label{fig:tiles}
\end{figure}
\subsection{Reporting individual components}
\begin{minipage}[t]{.47\linewidth}
\small\textbf{Quantitative evidence.} Keep precision consistent within each metric. Explain the arrows, identify the evaluation split and report the sample count. 
\end{minipage}\hfill
\begin{minipage}[t]{.47\linewidth}
\small\textbf{Qualitative evidence.} Use matched prompts, aligned frame times and a common crop policy. Disclose how examples were selected.
\end{minipage}
\vspace{4mm}
\begin{fxcallout}{Evidence before emphasis}
The light green row is a visual example of a highlighted method. It does not imply that the method outperforms the baselines. Insert verified data before assigning any best-result formatting.
\end{fxcallout}


==> sections_pre/method.tex <==
\fxkicker{Context / formulation / mechanism}
\section{Related Work}
Organize prior work by the question it answers. Place the closest baseline next to the proposed approach to locate the contribution. The numeric citation style compresses adjacent references automatically~\cite{yin2024dmd2,gao2025seedance}.
\section{Methodology}
\subsection{Overview}
Introduce the input, output and learnable components before presenting the objective. Figure~\ref{fig:pipeline} uses dark green for the main path, teal for weighting and gold for the objective.
\begin{figure}[htbp]
\centering
\fxfitfigure{\begin{tikzpicture}[x=1cm,y=1cm,>=Stealth,font=\sffamily\footnotesize,
box/.style={draw=FXLine,fill=FXPaper,rounded corners=2pt,minimum height=1.12cm,text width=2.6cm,align=center},arr/.style={->,line width=.75pt,FXForest}]
\node[box] (s) at (1.5,0) {Student generator\\$G_\theta$};
\node[box] (v) at (5.2,0) {Generated rollout\\$\mathbf{V}$};
\node[box,draw=FXForest,fill=FXPale] (r) at (9.0,0) {Shared reward\\model};
\node[box,draw=FXTeal,fill=FXTeal!6] (w) at (12.7,0) {Rollout / region\\weights};
\draw[arr] (s)--(v);\draw[arr] (v)--(r);\draw[arr] (r)--(w);
\node[box,text width=5.2cm,fill=FXGold!12,draw=FXGold] (l) at (7.1,-2.0) {Weighted distillation objective};
\draw[arr] (v.south)--++(0,-.55)-|(l.north);
\draw[arr] (w.south)--++(0,-1.44)--(l.east);
\draw[arr,dashed] (l.west)-|(s.south);
\node[font=\sffamily\scriptsize,text=FXMuted] at (2.5,-2.3) {training update};
\end{tikzpicture}}
\caption{Conceptual layout inspired by Stream-R1. This simplified diagram demonstrates the template's figure styling; it is not a complete implementation graph.}\label{fig:pipeline}
\end{figure}
\subsection{Notation and objective}
Define each symbol at first use and state the domain over which an average is taken. The expressions below demonstrate rollout reweighting and a general weighted reduction:
\begin{align}
w_{\mathrm{inter}} &= \exp\!\left(\beta r_{\mathrm{final}}\right),\label{eq:weight}\\
\mathcal{L} &= w_{\mathrm{inter}}\,\frac{1}{|\Omega|}\sum_{i\in\Omega} W_{\mathrm{intra},i}\,\ell_i.\label{eq:objective}
\end{align}
Equation~\eqref{eq:weight} follows the source weighting rule; Eq.~\eqref{eq:objective} is schematic notation for the layout specimen. In a complete method section, specify normalization, gradient flow, numerical stabilization and the exact definition of the elementwise loss.
\subsection{Training procedure}
\begin{fxcallout}{Algorithm 1\quad Example structure for pseudocode}
\textbf{Input:} training prompts, model parameters and optimizer settings.\par
\begin{enumerate}[nosep]
\item Construct the batch and compute the required model outputs.
\item Evaluate the objective, specifying all detached quantities.
\item Update trainable parameters and record the evaluation statistics.
\end{enumerate}
\textbf{Output:} the trained model and a reproducible configuration.
\end{fxcallout}


==> variant-A.tex <==
\PassOptionsToClass{fontA}{framexpaper}
\input{main.tex}


==> variant-B.tex <==
\PassOptionsToClass{fontB}{framexpaper}
\input{main.tex}


==> variant-C.tex <==
\PassOptionsToClass{fontC}{framexpaper}
\input{main.tex}


==> variant-D.tex <==
\PassOptionsToClass{fontD}{framexpaper}
\input{main.tex}

